Searching for Two-Stream Models in Multivariate Space for Video Recognition

Conventional video models rely on a single stream to capture the complex spatial-temporal features. Recent work on two-stream video models, such as SlowFast network and AssembleNet, prescribe separate streams to learn complementary features, and achieve stronger performance. However, manually designing both streams as well as the in-between fusion blocks is a daunting task, requiring to explore a tremendously large design space. Such manual exploration is time-consuming and often ends up with sub-optimal architectures when computational resources are limited and the exploration is insufficient. In this work, we present a pragmatic neural architecture search approach, which is able to search for two-stream video models in giant spaces efficiently. We design a multivariate search space, including 6 search variables to capture a wide variety of choices in designing two-stream models. Furthermore, we propose a progressive search procedure, by searching for the architecture of individual streams, fusion blocks, and attention blocks one after the other. We demonstrate two-stream models with significantly better performance can be automatically discovered in our design space. Our searched two-stream models, namely Auto-TSNet, consistently outperform other models on standard benchmarks. On Kinetics, compared with the SlowFast model, our Auto-TSNet-L model reduces FLOPS by nearly 11 times while achieving the same accuracy 78.9%. On Something-Something-V2, Auto-TSNet-M improves the accuracy by at least 2% over other methods which use less than 50 GFLOPS per video.

==> tex/4_2_cost_aware_not_used.tex <==
\subsection{Cost-Aware Search}

 We extend PARSEC to support cost-aware search where a target model FLOPS is chosen before the search starts. During the search, any model uses FLOPS more than that will be penalized. Such cost-aware search allows to search models with a target FLOPS, not only facilitating the comparisons with other SOTA models using a similar amount of compute, but also adapting the search to compute-sensitive scenarios, such as searching compact models for mobile applications. More details on cost-aware search can be seen in the supplement.

% \Heng{Is the cost-aware search our major contribution? If so, can we do some analysis to demonstrate its advantage? Such as does it converge faster? does the searched backbone make more sense?}


% Formally, the architecture parameters $\alpha$ define the architecture distribution, and the model weights in building blocks are denoted as $\omega$. For training videos $\mathbf{X}$ with groundtruth labels $\mathbf{y}$, we define the cost-aware search loss as below.

% \begin{equation}
%     \mathcal{L}(\mathbf{\alpha}, \omega) = -\textup{log}\;P(\mathbf{y} | \textbf{X}, \omega, \mathbf{\alpha}) + \beta\;\textup{log}\;C(\mathbf{\alpha})
% \end{equation}

% \begin{equation}
% \begin{align*}
%     \mathcal{L}(\mathbf{\alpha}, \omega) &= -\textup{log}\;P(\mathbf{y} | \textbf{X}, \omega, \mathbf{\alpha}) + \beta\;\textup{log}\;C(\mathbf{\alpha})
% \end{align*}
% \label{eqn:hinge-loss-cost}
% \end{equation}
% \vspace{-0.2cm}

% Both the negative data likelihood $P(\mathbf{y} | \textbf{X}, \omega, \mathbf{\alpha})$ and the  architecture cost $C(\mathbf{\alpha})$ can be approximated by sampling $K$ architectures $\{\mathbf{A}_k\}$ at each search step, and the hinge cost for a sampled architecture is $C(\mathbf{A}_k) = max(0, \frac{\textup{FLOPS}(\mathbf{A}_k)}{\textup{TAR}} - 1)$, $\beta$ denotes the coefficient of architecture cost. More background details on PARSEC can be seen in supplement.


